Students' interest in knowledge acquisition in Artificial Intelligence

Some students' expectations and points of view related to the Artificial Intelligence course are explored and analyzed in this study. We anonymous collected answers from 58 undergraduate students out of 200 enrolled in the Computer Science specialization. The answers were analysed and interpreted using thematic analysis to find out their interests and attractive and unattractive aspects related to the Artificial Intelligence study topic. We concluded that students are interested in Artificial Intelligence due to its trendiness, applicability, their passion and interest in the subject, the potential for future growth, and high salaries. However, the students' expectations were mainly related to achieving medium knowledge in the Artificial Intelligence field, and men seem to be more interested in acquiring high-level skills than women. The most common part that wasn't enjoyed by the students was the mathematical aspect used in Artificial Intelligence. Some of them (a small group) were also aware of the Artificial Intelligence potential which could be used in an unethical manner for negative purposes. Our study also provides a short comparison to the Databases course, in which students were not that passionate or interested in achieving medium knowledge, their interest was related to DB usage and basic information.

==> PROCS_KES2023_LATEX_Template/plan.tex <==
2.5 -3 pagini Raspuns la intrebari
1 pag referinte
1 conclusion+threads to validity
1 metodologia + participanti
1 abstract

2.5 - introd+literature


Pt site-ul de la KES2023
User ID = k23-132
Password = MWTF2719


% \bibitem{Ahmed2020}
%Zeeshan Ahmed, Khalid Mohamed, Saman Zeeshan, and XinQi Dong. (2020) ``Artificial intelligence with multi-functional machine learning platform development for better healthcare and precision medicine" {\it Database - The Journal of Biological Databases and Curation} {\bf 2020}: 1--35.

%\bibitem{Aoun2017}
%Aoun, Joseph E. (2017) ``Robot-Proof: Higher Education in the Age of Artificial Intelligence" {\it The MIT Press, Cambridge, Massachusetts, London, England}. 

%\bibitem{Dogan2023}
%Murat Ertan Dogan, Tulay Goru Dogan, and Aras Bozkurt. (2023) ``The Use of Artificial Intelligence (AI) in Online Learning and Distance Education Processes: A Systematic Review of Empirical Studies" {\it MDPI, Applied Sciences} {\bf 13} (5): 3056--3068.

%\bibitem{Fesharaki2011}
%M. Fesharaki, Hossein Shirazi, and A. Bakhshi. (2011) ``Knowledge acquisition from database of information management and documentation softwares by data mining techniques" {\it Learning from Dynamic Systems. Knowledge Management and Knowledge Engineering} {\bf 26}: 259-283.

%\bibitem{Holder2006}
% Lawrence B. Holder, Zdravko Markov, and Ingrid Russell. (2006) ``Advances in Knowledge Acquisition and Representation" {\it International Journal on Artificial Intelligence Tools} {\bf 15} (6): 867--874.

%\bibitem{Hunter1990}
%L. Hunter. (1990) ``Knowledge acquisition planning for inference from large databases" {\it Nat. Libr. of Med., Bethesda, MD, USA, Twenty-Third Annual Hawaii International Conference on System Sciences} {\bf 2}: 35--44.

%\bibitem{Hsu12}
%Donald Hsu. (2012) ``Case Studies in Systems and Database Courses" {\it E-Leader Berlin}.

%\bibitem{Kidd1987}
%Alison L. Kidd. (1987) ``Knowledge Acquisition" {\it In: Knowledge Acquisition for Expert Systems: A Practical Handbook. Springer US, Boston, MA}: 1--16.

%\bibitem{Kleiner1996}
%M.S. Kleiner, and S.A. Carey. (1996) ``Knowledge acquisition in support of artificial intelligence: an example and some lessons learned" {\it Proceedings Winter Simulation Conference}: 884--891.

%\bibitem{Kobayashi1991}
%S. Kobayashi and R. Mizoguch. (1991) ``Knowledge acquisition and learning for expert systems: Research activities in Japan" {\it IFAC Proceedings Volumes} {\bf 24} (11): 253-258.

%\bibitem{icsoft22} 
%Manuela Andreea Petrescu, and Adrian Sterca. (2022) ``Agile methodology in online learning and how it can improve communication. A case study" {\it In Proceedings of the 17th International Conference on Software Technologies}: 542--549.

% \bibitem{Rahmani2021}
% A.M. Rahmani, E. Azhir, S. Ali, m. Mohammadi, O.H. Ahmed OH, M. Yassin Ghafour, S. Hasan Ahmed, and M. Hosseinzade. (2021) ``Artificial intelligence approaches and mechanisms for big data analytics: a systematic study" {\it PeerJ Comput Sci.} {'bf 7}: 488.

%\bibitem{Sarker2021}
%Iqbal H. Sarker. (2021) ``Deep Learning: A Comprehensive Overview on Techniques, Taxonomy, Applications and Research Directions" {\it SN Computer Science, Springer Nature Journal} {\bf 2}: 420--440.

%\bibitem{Uzun20}
%Adem Uzun, Ahmet Onur, and Sercan Alabay. (2020) ``Students’ views on database management systems course designed according to problem-based learning" {\it International Journal of Evaluation and Research in Education (IJERE)} {\bf 9}: 177.

%\bibitem{Taipalus20}
%Toni Taipalus, and Ville Seppänen. (2020) ``SQL Education: A Systematic Mapping Study and Future Research Agenda" {\it ACM Transactions on Computing Education} {\bf 20} (3):1--33.

%\bibitem{Wayne1989}
%A. Nelson Wayne (1989) ``Artificial intelligence knowledge acquisition techniques for instructional development" {\it Educational Technology Research and Development} {\bf 37}: 81--94.

==> plan.tex <==
2.5 -3 pagini Raspuns la intrebari
1 pag referinte
1 conclusion+threads to validity
1 metodologia + participanti
1 abstract

2.5 - introd+literature


Pt site-ul de la KES2023
User ID = k23-132
Password = MWTF2719


% \bibitem{Ahmed2020}
%Zeeshan Ahmed, Khalid Mohamed, Saman Zeeshan, and XinQi Dong. (2020) ``Artificial intelligence with multi-functional machine learning platform development for better healthcare and precision medicine" {\it Database - The Journal of Biological Databases and Curation} {\bf 2020}: 1--35.

%\bibitem{Aoun2017}
%Aoun, Joseph E. (2017) ``Robot-Proof: Higher Education in the Age of Artificial Intelligence" {\it The MIT Press, Cambridge, Massachusetts, London, England}. 

%\bibitem{Dogan2023}
%Murat Ertan Dogan, Tulay Goru Dogan, and Aras Bozkurt. (2023) ``The Use of Artificial Intelligence (AI) in Online Learning and Distance Education Processes: A Systematic Review of Empirical Studies" {\it MDPI, Applied Sciences} {\bf 13} (5): 3056--3068.

%\bibitem{Fesharaki2011}
%M. Fesharaki, Hossein Shirazi, and A. Bakhshi. (2011) ``Knowledge acquisition from database of information management and documentation softwares by data mining techniques" {\it Learning from Dynamic Systems. Knowledge Management and Knowledge Engineering} {\bf 26}: 259-283.

%\bibitem{Holder2006}
% Lawrence B. Holder, Zdravko Markov, and Ingrid Russell. (2006) ``Advances in Knowledge Acquisition and Representation" {\it International Journal on Artificial Intelligence Tools} {\bf 15} (6): 867--874.

%\bibitem{Hunter1990}
%L. Hunter. (1990) ``Knowledge acquisition planning for inference from large databases" {\it Nat. Libr. of Med., Bethesda, MD, USA, Twenty-Third Annual Hawaii International Conference on System Sciences} {\bf 2}: 35--44.

%\bibitem{Hsu12}
%Donald Hsu. (2012) ``Case Studies in Systems and Database Courses" {\it E-Leader Berlin}.

%\bibitem{Kidd1987}
%Alison L. Kidd. (1987) ``Knowledge Acquisition" {\it In: Knowledge Acquisition for Expert Systems: A Practical Handbook. Springer US, Boston, MA}: 1--16.

%\bibitem{Kleiner1996}
%M.S. Kleiner, and S.A. Carey. (1996) ``Knowledge acquisition in support of artificial intelligence: an example and some lessons learned" {\it Proceedings Winter Simulation Conference}: 884--891.

%\bibitem{Kobayashi1991}
%S. Kobayashi and R. Mizoguch. (1991) ``Knowledge acquisition and learning for expert systems: Research activities in Japan" {\it IFAC Proceedings Volumes} {\bf 24} (11): 253-258.

%\bibitem{icsoft22} 
%Manuela Andreea Petrescu, and Adrian Sterca. (2022) ``Agile methodology in online learning and how it can improve communication. A case study" {\it In Proceedings of the 17th International Conference on Software Technologies}: 542--549.

% \bibitem{Rahmani2021}
% A.M. Rahmani, E. Azhir, S. Ali, m. Mohammadi, O.H. Ahmed OH, M. Yassin Ghafour, S. Hasan Ahmed, and M. Hosseinzade. (2021) ``Artificial intelligence approaches and mechanisms for big data analytics: a systematic study" {\it PeerJ Comput Sci.} {'bf 7}: 488.

%\bibitem{Sarker2021}
%Iqbal H. Sarker. (2021) ``Deep Learning: A Comprehensive Overview on Techniques, Taxonomy, Applications and Research Directions" {\it SN Computer Science, Springer Nature Journal} {\bf 2}: 420--440.

%\bibitem{Uzun20}
%Adem Uzun, Ahmet Onur, and Sercan Alabay. (2020) ``Students’ views on database management systems course designed according to problem-based learning" {\it International Journal of Evaluation and Research in Education (IJERE)} {\bf 9}: 177.

%\bibitem{Taipalus20}
%Toni Taipalus, and Ville Seppänen. (2020) ``SQL Education: A Systematic Mapping Study and Future Research Agenda" {\it ACM Transactions on Computing Education} {\bf 20} (3):1--33.

%\bibitem{Wayne1989}
%A. Nelson Wayne (1989) ``Artificial intelligence knowledge acquisition techniques for instructional development" {\it Educational Technology Research and Development} {\bf 37}: 81--94.
